Language Representations Can be What Recommenders Need: Findings and Potentials

Recent studies empirically indicate that language models (LMs) encode rich world knowledge beyond mere semantics, attracting significant attention across various fields. However, in the recommendation domain, it remains uncertain whether LMs implicitly encode user preference information. Contrary to prevailing understanding that LMs and traditional recommenders learn two distinct representation spaces due to the huge gap in language and behavior modeling objectives, this work re-examines such understanding and explores extracting a recommendation space directly from the language representation space. Surprisingly, our findings demonstrate that item representations, when linearly mapped from advanced LM representations, yield superior recommendation performance. This outcome suggests the possible homomorphism between the advanced language representation space and an effective item representation space for recommendation, implying that collaborative signals may be implicitly encoded within LMs. Motivated by these findings, we explore the possibility of designing advanced collaborative filtering (CF) models purely based on language representations without ID-based embeddings. To be specific, we incorporate several crucial components to build a simple yet effective model, with item titles as the input. Empirical results show that such a simple model can outperform leading ID-based CF models, which sheds light on using language representations for better recommendation. Moreover, we systematically analyze this simple model and find several key features for using advanced language representations: a good initialization for item representations, zero-shot recommendation abilities, and being aware of user intention. Our findings highlight the connection between language modeling and behavior modeling, which can inspire both natural language processing and recommender system communities.

==> chapters/1_introduction.tex <==
\section{Introduction}
\begin{figure*}[t]
     \centering
    \begin{subfigure}[b]{0.98\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/intro/linear_trans.png}
         % \includegraphics[width=\textwidth]{figures/intro/intro_compare.png}
         \caption{Linearly mapping language representations into the recommendation space}
         \label{fig:linear-mapping}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         % \includegraphics[width=\textwidth]{figures/intro/linear-mapping.png}
         \includegraphics[width=\textwidth]{figures/intro/intro_compare.png}
         \caption{Performance comparison}
         \label{fig:linear-performance}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.66\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/intro/intro-tSNE.png}
         \caption{\za{The t-SNE representations of movies and user intention in two spaces.}}
         % The t-SNE visualization of items representations}
         \label{fig:tsne-intro}
     \end{subfigure}
    \vspace{-5pt} 
  \caption{
  Linearly mapping item titles in language representation space into recommendation space yields superior recommendation performance on Movies \& TV \citep{Amazon} dataset.
  (\ref{fig:linear-mapping}) The framework of linear mapping.
  (\ref{fig:linear-performance}) The recommendation performance comparison between leading CF recommenders and linear mapping.
  (\ref{fig:tsne-intro}) The t-SNE \citep{tsne} visualizations of movie representations, with colored lines linking identical movies or user intention across language space (left) and linearly projected recommendation space (right).
  }
  \label{fig:intro}
        \vspace{-15pt}
\end{figure*}

Language models (LMs) have achieved great success across various domains \citep{transformer, Bert, Llama3, GPT4}, raising a critical question about the knowledge encoded within \slh{their} language representation spaces.
Recent studies empirically find that LMs extend beyond semantic understanding to encode comprehensive world knowledge about various domains, such as game states \citep{board-game-linear}, lexical attributes \citep{lex-linear}, and even concepts of space and time \citep{space-and-time} through language modeling.
However, in the domain of recommendation where the integration of LMs is attracting widespread interest \citep{Rec-LLM-era, LLM4GenRec, Survey-LLM4Rec}, it remains unclear whether LMs inherently encode relevant information on user preferences and behaviors in their representation spaces.
% \slh{One possible reason for this lies in the significant difference between the objectives of language modeling for LMs and user behavior modeling for recommenders \citep{TALLRec, LLaRA, CLLMRec, LC-Rec}.}

Currently, one prevailing understanding holds that general LMs and traditional recommenders encode distinct representation spaces --- one for language modeling and the other for user behavior modeling --- but they offer potentials to enhance each other in downstream recommendation tasks
% (due to the difference between language modeling and user behavior modeling): the language space and the recommendation space (\ie user and item representation space), but each offers potentials to enhance the other for recommendation tasks 
\citep{CoLLM}.
On the one hand, when using LMs as recommenders, aligning the language space with the recommendation space can significantly improve the performance \citep{How-can-benefit, ImpactLLM, Prompt4Rec}.
Various alignment strategies are proposed, including fine-tuning LMs with recommendation data \citep{InstructRec, TALLRec, P5, M6-Rec, ReLLa}, incorporating embeddings from traditional recommenders as a new modality of LMs \citep{LLaRA, CoLLM, Recinterpreter}, and extending the vocabulary of LMs with item tokens \citep{CLLMRec, LC-Rec, TIGER, trillion-param-genrec}.
On the other hand, when using LMs as the enhancer, traditional ID-based recommenders greatly benefit from leveraging text representations \citep{TenRec, where-to-go, TCF, BLAIR}, semantic and reasoning information \citep{LLMRec, RLMRec, KAR}, and generated user behaviors \citep{Agent4Rec, AgentCF}. \za{Despite these efforts, explicit studies of the relationship between language and recommendation spaces remain largely unexplored.}
% On the other hand, when using LMs as the enhancer, traditional recommenders greatly benefit from \za{from} leveraging text representations \citep{TenRec, NineRec, where-to-go, TCF, modality-all-you-need, UniSRec, ZESRec, Recformer, BLAIR, VQ-Rec, UniTRec, U-Bert, WhiteningRec, PeterRec}, semantic and reasoning information \citep{LLMRec, RLMRec, KAR, BAHE}, and generated user behaviors \citep{Agent4Rec, AgentCF}. \za{Despite these efforts, explicit studies of the relationship between language and recommendation spaces remain largely unexplored.}

In this work, we rethink the prevailing understanding and explore whether LMs have inherently encoded user preferences solely through language modeling.
Specifically, we test the possibility of directly deriving a recommendation space from the language representation space, assessing whether the representations of item textual metadata (\eg titles) obtained from LMs can \za{independently} achieve satisfactory recommendation performance.
Positive results would imply that user behavioral patterns, such as \textbf{collaborative signals} 
% (\ie \slh{user} preference similarities between items) 
(\ie users' preference similarities reflected by their behavioral similarities)
\citep{NGCF, POI-cf-signals}, \slh{may} be implicitly encoded by LMs.
To test this hypothesis, we employ linear mapping \cite{linear-image-text} to project the language representations of item titles into a recommendation space (see Figure \ref{fig:linear-mapping}).
\za{According to the empirical results of linear mapping, our observations include:}
\begin{itemize} [leftmargin = *]
    \item 
    % Semantic textual similarities (STS) \citep{MTEB} 
    % may also reflect user preference similarities 
    \iclr{Before linear mapping, language representation similarities (\ie semantic textual similarities (STS) \citep{MTEB}) may reflect user preference similarities for item contents.}
    (see Figure \ref{fig:tsne-intro}). For example, movies with themes of superheroes and monsters cluster together in both language and recommendation spaces.
    % \item Language representations encode user preference similarities beyond STS. 
    \item
    % Surprisingly, this simple linear mapping yields high-quality item representations, 
    \iclr{After linear mapping, language representations are transformed into high-quality item representations}, which achieve exceptional recommendation performance (see Figure \ref{fig:linear-performance} and experimental results in Section \ref{sec:linear-result}). Moreover, the performance improves as the language model size increases and remains relatively robust to prompt disturbances (see Section \ref{sec:linear-result}).
    % language representations perform better in linear mapping as the language model size increases, and are fairly robust to the disturbance in the prompt.
    \item \iclr{Post-mapping language representations encode user preference similarities beyond STS. }
    For instance, while certain movies, such as those of homosexual movies (illustrated in Figure \ref{fig:tsne-intro}), show low STS and their representations disperse in the language space, their projections through linear mapping tend to cluster together, reflecting high user preference similarities.
    % Interestingly, the linear mapping effectively reveals preference similarities that may be implicit or even obscure in the language space. 
    % For instance, while certain movies, \za{such as those of homosexual movies (illustrated in Figure \ref{fig:tsne-intro})}, show dispersed representations in the language space, their projections through linear mapping tend to cluster together, reflecting their \za{genres affiliation}.
    % This phenomenon underscores the potential of linear mapping to uncover underlying patterns in data that are not immediately apparent from language-based representations alone.
\end{itemize}


These findings suggest the \textbf{homomorphism} \citep{homomorphism} between the language representation space of advanced LMs and an effective item representation space for recommendation.
% \za{Motivated by this insight,} we propose a new \za{language-representation-based} recommendation paradigm for general collaborative filtering (CF), which \za{utilizes} the pre-trained language representations of item titles as the item input and the average historical \za{interactions'} representations as the user input. 
% Different from traditional ID-based CF models \citep{MF, LightGCN, NGCF} that heavily rely on \za{trainable} user and item IDs, this paradigm solely uses pre-trained LM embeddings and completely abandons ID-based embeddings. 
\slh{Motivated by this insight, we explore the possibility of building advanced collaborative filtering (CF) models based solely on language representations.} To be specific, we design a simple model architecture consisting of several crucial components: a two-layer MLP with graph convolution, and the popular contrastive loss, InfoNCE \citep{InfoNCE, Sampled_Softmax}, as the objective function. 
% In this paper, to fully explore the potential of advanced language representations, we adopt a simple \za{model architecture consisting of a two-layer MLP with graph convolution}, and \za{the popular contrastive loss,} InfoNCE \citep{InfoNCE, Sampled_Softmax, Rendle-implicit}, as the \za{objective} function. 
We term this model AlphaRec for its simplicity and a series of good properties. 
% To our surprise, we empirically find out 
Surprisingly, our empirical results show that such a simple model with embeddings from pre-trained LMs can outperform leading ID-based CF models on multiple datasets. 
This result sheds light on using language representations for better recommendation.
% This model is named AlphaRec for its originality, a series of good properties, and an adjustable hyperparameter $\alpha$ for user intention capture. 

Furthermore, we systematically analyze this simple model and discover several potentials of adopting language representations for recommendation. First, language representations may serve as a good initialization for item representations, with few adjustments to achieve high recommendation performance (see Section \ref{sec:convergence}). 
% to become excellent item representations for recommendation (see Section \ref{sec:convergence}). 
This is evidenced by the rapid training convergence of AlphaRec. 
Second, advanced language representations provide strong zero-shot recommendation capability across entirely new datasets (see Section \ref{sec:zero-shot}). 
% By co-training on three Amazon datasets (Books, Movies \& TV, and Video Games) \citep{Amazon}, AlphaRec can achieve performance comparable to the fully-trained LightGCN on entirely different platforms (MovieLens-1M \citep{MovieLens} and BookCrossing \citep{BookCrossing}), and even exceed LightGCN in a completely new domain (Amazon Industrial), without additional training on these target datasets.
% This capability underscores the potential for advanced language representations to develop more general recommenders.
By co-training on multiple datasets, AlphaRec can achieve performance comparable to or even surpassing the fully-trained LightGCN \citep{LightGCN} on new datasets without additional training. This underscores the potential for adopting advanced language representations to develop more generalizable recommenders.
% (MovieLens-1M \citep{MovieLens} and BookCrossing \citep{BookCrossing}), and even exceed LightGCN in a completely new domain (Amazon Industrial), without additional training on these target datasets.
% This capability underscores the potential for advanced language representations to develop more general recommenders.
Third, advanced language representations provide opportunities for perceiving user intentions to refine recommendation results (see Section \ref{sec:search}).
% AlphaRec is user-friendly, offering a \za{new} research paradigm that \za{enhances recommendation by leveraging language-based} user feedback (see Section \ref{sec:search}). 
Endowed with the inherent semantic comprehension of language representations, AlphaRec can adjust recommendations according to text-based user intentions, enabling recommenders to evolve into intention-aware systems through a straightforward paradigm shift.

\iclr{
In total, we summarize the contributions and key findings of this paper as follows:
\begin{itemize}[leftmargin=*]
    \item 
    % As far as we know, this is the first work to study the relationship between language spaces and recommendation spaces from the perspective of linear mapping. 
    % With linear mapping, we empirically reveal the possible homomorphism between two spaces for the first time.
    With linear mapping, we empirically reveal the possible homomorphism between language spaces and recommendation spaces for the first time.
    \item We explore the power of advanced language representations for recommendation and develop a simple yet effective model called AlphaRec. 
    % We find out that, 
    With such a simple model design, recommenders solely based on language representations can outperform leading ID-based CF models.
    \item We discuss and highlight the potentials of adopting advanced language representations: good initialization for item representations, zero-shot ability, and intention-aware ability.
\end{itemize}
}







==> chapters/2_preliminary.tex <==
\section{Preliminary}
\iclr{
\subsection{Task Formulation}

% Personalized item recommendation aims to recommend items that maximize the reward (\eg click, buy) of users \citep{DIN}. 
Personalized recommendation aims to learn user preferences from historical interactions with items (\eg view, click, purchase) and find items of interest \citep{DIN}. 
% # Find items of interest
In this paper, we adopt one common recommendation setting: collaborative filtering (CF) \citep{Rendle-Advance_CF}.
CF aims to select item $i \in \mathcal{I}$ that best matches user $u$'s preferences based on binary interaction data $\mathbf{Y} = [y_{ui}]$, where $y_{ui} = 1$ indicates user $u \in \mathcal{U}$ has interacted with item $i$, and $y_{ui} = 0$ otherwise \citep{Rendle-implicit}. 
% To be different: and $y_{ui} = 0$ otherwise 
% The primary objective of CF
A common paradigm of CF models is to model the user-item interaction matrix $\mathbf{Y}$ using a scoring function $\hat{y}: \mathcal{U} \times \mathcal{I} \rightarrow \mathbb{R}$, where $\hat{y}_{ui}$ predicts user $u$'s preference for item $i$. 
% Typically is used to summarize our definition
Typically, the scoring function is defined as $\hat{y}_{ui} = s \circ \phi_\theta(\mathbf{x}_u, \mathbf{x}_i)$, involving three key components: pre-existing features $\mathbf{x}_u$ and $\mathbf{x}_i$ for user $u$ and item $i$, a recommendation representation learning module $\phi_\theta(\cdot,\cdot)$ parameterized by $\theta$, and a similarity function $s(\cdot,\cdot)$.
The recommendation representation learning module $\phi_\theta$ transfers $\mathbf{x}_u$ and $\mathbf{x}_i$ into final representations $\mathbf{e}_u$ and $\mathbf{e}_i$ for similarity matching $s(\cdot,\cdot)$, and the Top-$K$ highest scoring items are recommended to $u$. 
The architecture of recommendation representation learning $\phi_\theta$ can vary widely, including ID-based embedding matrices \citep{MF}, multilayer perceptions \citep{NCF}, graph neural networks \citep{NGCF, LightGCL}, and variational autoencoders \citep{MultVAE}.
For the similarity function, it measures the similarity between users and items in the recommendation representation space. In this paper, we adopt the widely used similarity function, cosine similarity \citep{, Adap-tau, Sampled_Softmax} $s(\mathbf{e}_u, \mathbf{e}_i) = \frac{\Trans{\mathbf{e}_{u}}\mathbf{e}_{i}}{\norm{\mathbf{e}_{u}}\cdot\norm{\mathbf{e}_{i}}}$ by default.
% Specifically, the recommender $\phi_\theta$ transfers the user and item into representations $\mathbf{e}_{u}$ and $\mathbf{e}_{i}$ for similarity matching. 
% For user $u$, items with the Top-$K$ highest score $s(\mathbf{e}_{u},\mathbf{e}_{i})$ are recommended. 
}



\iclr{
\subsection{Item Representation Generation}
% As the first step of CF models, item representation generation denotes how to get pre-existing item representations $\mathbf{x}_i$ as the input. It is crucial since it determines the model paradigm.
Here, we emphasize the critical role of item representation learning, which involves transforming item $i$'s pre-existing features $\mathbf{x}_i$ into representations $\mathbf{e}_i$ suitable for recommendation. This process is essential, as the quality of these representations directly impacts the recommendation performance.
% Different recommenders employ various methods for pre-existing item representations $\mathbf{x}_i$ generation. 
In this paper, we focus on two kinds of item representation generation \slh{according to the difference in pre-existing features $\mathbf{x}_i$}: ID-based generator and LM-based generator. 

\textbf{ID-based generator.}
 % and representation learning architecture $\phi_\theta(\cdot, \cdot)$.
Prevailing CF models \citep{LightGCN, SASRec} tend to adopt an ID-based paradigm. 
This paradigm usually transfers the ID information of each item $i$ as a one-hot encoding (\ie pre-existing features $\mathbf{x}_i$).
Then, it applies \slh{ID-based embedding matrices} to the sparse one-hot encoding to create dense and learnable embedding, 
% (\ie recommendation representation $\mathbf{e}_i$).
\slh{which are then transformed into ID-based item representations $\mathbf{e}_i$ using specific model structures. }
Optimizing the learning of ID-based representations allows us to effectively capture user preferences, leading to strong recommendation performance while maintaining low training and inference costs \citep{XSimGCL}.
% These models use the ID-based generator to assign one-hot vectors as pre-existing features $\mathbf{x}_i$ for items. 
% The ID-based generator exhibits excellent recommendation capabilities with low training and inference costs \cite{LightGCL, BC-loss}. 
However, it suffers several problems like poor domain transferability and lack of user intention-aware abilities, since one-hot vectors lack sufficient semantics beyond being identifiers \citep{LightGCN}.
% However, it suffers several problems like domain transferring and user intention-aware abilities, since one-hot vectors do not have any semantics beyond being identifiers \citep{LightGCN}. 

\textbf{LM-based generator.}
% usually > offen
LM-based generators are often used in content-based recommendation models \citep{YouTubeDNN}, where the pre-existing features $\mathbf{x}_i$ are extracted from the latent space of LMs. 
\slh{These features $\mathbf{x}_i$ are then fed into the model to obtain final item representations $\mathbf{e}_i$.} 
% We comprehensively 
% \slh{LM-based generators have shown effective in scenarios where the effectiveness of ID-based representations is insufficient (\eg cold start).} 
In this paper, we mainly focus on this kind of generator. 
For a comprehensive study, we consider both generative \citep{Llama2} and non-generative (\eg text embedding models \citep{MTEB}) LMs \slh{for pre-existing features extraction}, especially focusing on two popular model types: encoder-only models and decoder-only models. For encoder-only models, we include BERT-style models \citep{Bert, roberta}. For decoder-only models, we consider large language models (LLMs) \citep{Llama2}, and LLM-based embedding models \citep{OpenAI-CPT} (see Appendix \ref{apdx:used-LMs} for details about used LMs). 

\subsection{Evaluation Metrics}
To quantitatively measure the recommendation performance with various generators, we select three widely used metrics in recommendation in this paper: Hit Ratio (HR@$K$), Recall@$K$, Normalized Discounted Cumulative Gain (NDCG@$K$)), with $K$ set by default at 20. 
}

==> chapters/3_uncovering.tex <==
\iclr{
\section{Uncovering Collaborative Signals in LMs via Linear Mapping} \label{sec:linear-mapping}
% In Section \ref{sec:linear-objective}, we introduce the research objective and used method. In Section \ref{sec:linear-method}, we discuss the implementation details of linear mapping. In Section \ref{sec:linear-result}, we explore the existence and robustness of collaborative signals in language representations through empirical results.
This section elaborates on discovering collaborative signals encoded in language representations with linear mapping. In Section \ref{sec:linear-objective}, we first introduce the research objective. We then detail the implementation of the linear mapping in Section \ref{sec:linear-method}. Finally, in Section \ref{sec:linear-result}, we examine the existence and robustness of collaborative signals in language representations through empirical results.
\subsection{Objective} \label{sec:linear-objective}
% In this section, we aim to explore whether LMs implicitly encode user preference similarities in the representation spaces.
We investigate the following questions first: do LMs implicitly encode user preference similarities in their representation spaces? If so, can such encoded information increase with the size of LM and does it exist robustly? 
To achieve this, we use linear mapping to project language representations of item titles into a recommendation space and evaluate the properties of projected item representations. 
% Empirical results suggest the possible homomorphism \citep{homomorphism} between the representation spaces of advanced LMs and effective recommendation spaces.
\subsection{Linear Mapping} \label{sec:linear-method}
% Homomorphism \citep{homomorphism} is a mapping that preserves the structure between two vector spaces, ensuring consistency in operations (\eg addition). 
% Linear mapping .  
\slh{Linear mapping is one effective method for studying the representation properties of LMs} \citep{linear-image-text, Bengio-linear}, since it ensures the homomorphism \citep{homomorphism} between two vector spaces. However, such explorations in recommendation are still rare currently.
To linearly project representations from the language space into an item recommendation space, we adopt a trainable linear mapping matrix $\bm{W}$ as the representation learning module $\phi_\theta$. }
High performance of linear mapping on the test set would indicate the homomorphism between the language space and an effective recommendation space, suggesting the possible existence of collaborative signals 
% \slh{(\ie user preference similarities between items) \citep{LightGCN}}
in the language representation space \citep{linear-paradigm, space-and-time}. 
The overall framework of the linear mapping process is illustrated in Figure \ref{fig:linear-mapping}. 
Specifically, we use the language representations of item titles as pre-existing features $\mathbf{x}_i$. 
For initial user feature $\mathbf{x}_u$, we use the average of the title representations of historically interacted items, defined as $\mathbf{x}_{u} = \frac{1}{|\Set{N}_u|}\sum_{i\in\Set{N}_u}\mathbf{x}_{i}$, where $\Set{N}_u$ is the set of items user $u$ has interacted with.
Detailed procedures for obtaining these language-based features are provided in Appendix \ref{apdx:get-representations}.
% Please see more details about how we get language-representation-based $u,i$ embeddings in Appendix \ref{apdx:get-representations}.
The linear mapping matrix sets user and item representations as $\mathbf{e}_u=\bm{W}\mathbf{x}_u$ and $\mathbf{e}_i=\bm{W}\mathbf{x}_i$ respectively.
To learn the linear mapping matrix $\bm{W}$, we adopt the InfoNCE loss \citep{InfoNCE} as the objective function, which has demonstrated state-of-the-art performance in both ID-based \citep{AdvInfoNCE, XSimGCL} and LM-enhanced CF recommenders \citep{RLMRec} (refer to Equation \eqref{eq:InfoNCE} for the formula).

\subsection{Empirical Findings} \label{sec:linear-result}
\begin{table*}[t]
    \centering
    \caption{The recommendation performance of linear mapping comparing with classical ID-based CF baselines.}
    \label{tab:linear}
    \vspace{-5pt}
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{ll|ccc|ccc|ccc}
    \toprule
    % \multicolumn{1}{c}{} & \multicolumn{12}{c}{Tencent}      \\
    & & \multicolumn{3}{c|}{Movies \& TV}  & \multicolumn{3}{c|}{Video Games} & \multicolumn{3}{c}{Books} \\
    & \multicolumn{1}{c|}{} & Recall & NDCG & HR & Recall & NDCG & HR & Recall & NDCG & HR \\\midrule

\multirow{3}{*}{\rotatebox{90}{CF}} & MF \citep{BPR} & $0.0568$& $0.0519$ & $0.3377$ &$0.0323$ & $0.0195$ & $0.0864$ & $0.0437$ & $0.0391$ & $0.2476$  \\
& MultVAE \citep{MultVAE} & $0.0853$& $0.0776$ & $0.4434$ &$0.0908$ & $0.0531$ & $0.2211$ & $0.0722$ & $0.0597$ & $\underline{0.3418}$  \\
& LightGCN \citep{LightGCN} & $0.0849$& $0.0747$ & $0.4397$ &$0.1007$ & $0.0590$ & $0.2281$ & $0.0723$ & \underline{0.0608} & $\textbf{0.3489}$  \\\midrule
% Linear Mapping  & & & & & & & & &  \\
\multirow{7}{*}{\rotatebox{90}{Linear Mapping}} & BERT & 0.0415 & 0.0399 & 0.2362 & 0.0524 & 0.0309 & 0.1245 & 0.0226 & 0.0194 & 0.1240   \\
& RoBERTa  & 0.0406 & 0.0387 & 0.2277 & 0.0578 & 0.0338 & 0.1339 & 0.0247 & 0.0209 & 0.1262  \\
& Llama2-7B & 0.1027 & 0.0955 & 0.4952 & 0.1249 & 0.0729 & 0.2746 & 0.0662 & 0.0559 & 0.3176   \\
& Mistral-7B & 0.1039 & 0.0963 & 0.4994 & 0.1270 & 0.0687 & 0.2428 & 0.0650 & 0.0544 & 0.3124  \\
& text-embedding-ada-v2 & 0.0926 & 0.0874 & 0.4563 & 0.1176 & 0.0683 & 0.2579 & 0.0515 & 0.0436 & 0.2570  \\
& text-embeddings-3-large & \underline{0.1109} & \underline{0.1023} & \underline{0.5200} & \underline{0.1367} & \textbf{0.0793} & \textbf{0.2928} & \underline{0.0735} & \underline{0.0608} & 0.3355   \\
& SFR-Embedding-Mistral & \textbf{0.1152} & \textbf{0.1065} & \textbf{0.5327} & \textbf{0.1370} & \underline{0.0787} & \underline{0.2927} & \textbf{0.0738} & \textbf{0.0610} & 0.3371   \\
% \midrule
\bottomrule
\end{tabular}}
     \vspace{-5pt}
\end{table*} 

\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{0.31\textwidth}
      \centering
      \includegraphics[width=\textwidth]{figures/linear/scaling_movies.png}
      \caption{Movie \& TV}
  \end{subfigure}
  \begin{subfigure}[b]{0.305\textwidth}
      \centering
      \includegraphics[width=\textwidth]{figures/linear/scaling_games.png}
      \caption{Games}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
      \centering
      \includegraphics[width=\textwidth]{figures/linear/scaling_books.png}
      \caption{Books}
  \end{subfigure}
  \vspace{-5pt}
  \caption{The recommendation performance of linear mapping with different language model sizes.}\label{fig:scaling-effect}
  \vspace{-10pt}
\end{figure*}
\textbf{Existence. }
To verify the existence of collaborative signals in language representations, we test the recommendation performance of the linear mapping method and delve into the effect of linear mapping on the representation space. 
Table \ref{tab:linear} reports the recommendation performance yielded by the linear mapping on three Amazon datasets \citep{Amazon}, comparing with classic ID-based CF baselines: matrix factorization (MF) \citep{MF}, MultVAE \citep{MultVAE}, and LightGCN \citep{LightGCN} (see details about baselines in Appendix \ref{apdx:baselines-general}). Figure \ref{fig:tsne-intro} demonstrates the visualization of representations before and after linear mapping. We observe that:
\iclr{
\begin{itemize}[leftmargin = *]
    \item \textbf{Post-mapping representations of advanced LMs yield superior recommendation performance in most cases.} Both generative and non-generative LMs showcase excellent performance under the linear mapping setting. Moreover, with the advances in LMs, we observe that the performance of language representations exhibits a rising trend. Representations from early BERT-style models (\eg BERT \citep{Bert} and RoBERTa \citep{roberta}) only show weaker or equal capabilities compared with MF, failing behind LLMs largely. These results further suggest that, until very recently, the language representation spaces encode user preference similarities efficiently. 
    % The performance of most advanced text embedding models (\eg text-embeddings-3-large \citep{OpenAI-CPT} and SFR-Embedding-Mistral \citep{SFRAIResearch2024}) exceeds LightGCN on all datasets. 
    \item \textbf{Language representations encode user preference similarities beyond STS.} As illustrated in Figure \ref{fig:tsne-intro}, the textual meanings of homosexual movies vary dramatically. However, their post-mapping representations cluster together. This suggests that obscure user preference similarities may be implicitly encoded in the language representation space, and a simple linear mapping can reveal such preference similarities.
    % Figure \ref{fig:tsne-intro} suggests that obscure user preference similarities may be implicitly encoded in the language representation space. For example, the textual meanings of homosexual movies vary dramatically. However, their post-mapping representations cluster together. Linear mapping discovers their similar user preferences.
    \item \textbf{The linear mapping performance improves with the scaling of model size.} We conduct the linear mapping experiments on the Llama2 family \citep{Llama2}, varying the language model sizes (7B, 13B, and 70B). We do not choose Llama3 \citep{Llama3} since it does not provide models with a size of 13B. As illustrated in Figure \ref{fig:scaling-effect}, the linear mapping performance increases as the language model increases, indicating a rising trend in the encoded collaborative signals with the model size.
\end{itemize}
}
% In addition, with the help of linear mapping, for the first time, we are able to clearly quantify the gap in the representation spaces between different LMs for recommendation. 
% We also empirically show that these improvements may not merely come from the better feature encoding ability (refer to Appendix \ref{apdx:existence}). 

\begin{table*}[t]
    \centering
    \caption{The robustness of language representations for recommendation.}
    \label{tab:robustness}
    \vspace{-5pt}
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc}
    \toprule
    % \multicolumn{1}{c}{} & \multicolumn{12}{c}{Tencent}      \\
     & \multicolumn{3}{c|}{Movies \& TV}  & \multicolumn{3}{c|}{Video Games} & \multicolumn{3}{c}{Books}  \\
 & Recall & NDCG & HR & Recall & NDCG & HR & Recall & NDCG & HR \\\midrule
 Title + Random Noise & 0.0952 & 0.0887 & 0.4731 & 0.1213 & 0.0706 & 0.2722 & 0.0632 & 0.0525 & 0.3099   \\
 % Title + Metadata & 0.0924 & 0.0866 & 0.4679 & 0.1253 & 0.0733 & 0.2735 & 0.0653 & 0.0543 & 0.3104  \\
 Title Only & 0.1027 & 0.0955 & 0.4952 & 0.1249 & 0.0729 & 0.2746 & 0.0662 & 0.0559 & 0.3176   \\
% \midrule
\bottomrule
\end{tabular}}
     \vspace{-10pt}
\end{table*} 

\iclr{
\textbf{Robustness.} Another crucial question lies in whether the knowledge of recommendation exists robustly in language representations. To answer this question, we test the linear mapping performance under noisy prompts following previous works \citep{space-and-time}. 
Specifically, we compare two prompting strategies: a single title (Title Only. \eg Castlevania), and item title with 5-10 random letters (Title + Random Noise. \eg Castlevania sdfhdsk).
We report the results for Llama2-7B in Table \ref{tab:robustness}. We find that a slight disturbance on the oracle item title would not harm the performance of linear mapping much. 
This finding suggests the robustness of the recommendation knowledge encoded in the language representation space. 
}
% More interestingly, when adding additional metadata beyond item titles, which is widely adopted in previous studies \citep{KAR, RLMRec}, does not bring improvements in most cases and may even harm the linear mapping performance. This may indicate that the language model encodes rich world knowledge, being able to uniquely identify items using simple item titles.

% These findings suggest the possible homomorphism \citep{homomorphism} between language representation spaces of advanced LMs and effective item representation spaces for recommendation.
